Diverse Large-Scale ITS Dataset Created from Continuous Learning for Real-Time Vehicle Detection

In traffic engineering, vehicle detectors are trained on limited datasets resulting in poor accuracy when deployed in real world applications. Annotating large-scale high quality datasets is challenging. Typically, these datasets have limited diversity; they do not reflect the real-world operating environment. There is a need for a large-scale, cloud based positive and negative mining (PNM) process and a large-scale learning and evaluation system for the application of traffic event detection. The proposed positive and negative mining process addresses the quality of crowd sourced ground truth data through machine learning review and human feedback mechanisms. The proposed learning and evaluation system uses a distributed cloud computing framework to handle data-scaling issues associated with large numbers of samples and a high-dimensional feature space. The system is trained using AdaBoost on $1,000,000$ Haar-like features extracted from $70,000$ annotated video frames. The trained real-time vehicle detector achieves an accuracy of at least $95\%$ for $1/2$ and about $78\%$ for $19/20$ of the time when tested on approximately $7,500,000$ video frames. At the end of 2015, the dataset is expect to have over one billion annotated video frames.

==> backgroundproblems <==
Positive and Negative Mining:

DATASET:
Typically, bounding boxes or polygons are drawn around vehicles to localize them. Domain specific annotations such as vehicle class (e.g. passenger car, van, truck with trailer, bus) have not been observed in any of the data sets. In the new annotation tool, complex polygons allow for annotated objects to be tightly localized. Another significant problem with the datasets found is that they are limited in scope. In {}, {} and {}, a limited number of locations and perspectives are represented. Diverse weather conditions and lighting conditions are not necessarily present, and where they are, these conditions are not annotated. None of the datasets found annotate the roads or intersections to indicate lane geometries. {} is an example of a very diverse dataset, but the annotations provided are specifically for vehicle counting-type algorithms. Presence detection algorithms would likely require augmentation to the annotations.

The proposed dataset consists of detailed annotations for training and coarse or 'lo-fi' annotations for evaluation. Metrics such as countingi and presence detection may be defined. Data is annotated for weather conditions and visibility, allowing for targeted training and segmentation of evaluation results to expose failure modes.

Background survey

Koller's \cite{koller1998Image} dataset is NOT annotated! This dataset might be appropriate for an unsupervised approach.

Schneiderman and Kanade \cite{schneiderman2000Statistical} used 104 images containing 213 cars. Many of these images were of static vehicles, and they came from a variety of sources (print advertisements, stock photography, traffic cameras). The image annotations are very detailed, with wheels, lights, grills and windshields all being annotated. This type of annotated dataset is particularly useful for a feature engineering approach: lights, wheels, grills, etc are selected as the most significant features in detecting a car. The approach is to use these features and the known structural relationship between them to detect cars and their orientation in three-dimensional space. This type of data may not be as meaningful for a lower level approach, such as using combinations of haar wavelets to detect vehicles given a training set consisting of vehicles and non vehicles.

Papageorgiou \cite{papageorgiou2000CBCL} A dataset of 128x128 pixel images of the front or rear view of cars. The images are normalized so that bumpers are centred in the frame and are approximately 64 pixels wide. The data is not explicitly annotated, but the homogenous nature of the dataset allows for training on specific vehicle orientations. This dataset is not appropriate for oblique views of vehicles. There are 516 unique colour images of frontal or rear views of cars. These images, along with their mirrors are used to create a training set of sit 1032 positive samples. 5166 negative samples are used. It is not clear how the negative samples were chosen.

PETS 2001 \cite{makris2001Index} is a well known annotated dataset for training object detection algorithms. This training set was not assembled with any particular algorithm in mind. The dataset comes with tracking annotations.

Agarwal et al \cite{agarwal2004Learning} used a training set of 500 positive images, and 500 negative images in an annotated training set.

StreetScenes \cite{bileschi2006StreetScenes} is a database with very detailed annotations of vehicles, pedestrians, bicyles and backgrounds items such as sky, road, trees, buildings, stores and sidewalks in still images. Polygons are drawn tightly to objects (in contrast to unoriented bounding boxes found in many other annotated datasets.



